FMPC: Secure Multiparty Computation from Fourier Series and Parseval's Identity

FMPC is a novel multiparty computation protocol of arithmetic circuits based on secret-sharing, capable of computing multiplication of secrets with no online communication; it thus enjoys constant online communication latency in the size of the circuit. FMPC is based on the application of Fourier series to Parseval's identity, and introduces the first generalization of Parseval's identity for Fourier series applicable to an arbitrary number of inputs. FMPC operates in a setting where users wish to compute a function over some secret inputs by submitting the computation to a set of nodes, but is only suitable for the evaluation of low-depth arithmetic circuits. FMPC relies on an offline phase consisting of traditional preprocessing as introduced by established protocols like SPDZ, and innovates on the online phase that mainly consists of each node locally evaluating specific functions. FMPC paves the way for a new kind of multiparty computation protocols capable of computing multiplication of secrets as an alternative to circuit garbling and the traditional algebra introduced by Donald Beaver in 1991.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	main.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

==> sections/parseval.tex <==
% =========
% Parseval 
% =========
\section{Generalization of \parseval's Identity} \label{sec:generalized-parseval}
We present the generalization of \parseval's identity for \fourier series applicable to $n$ inputs. \parseval's identity traditionally applies only to two functions; we overcome this drawback by using the convolution operation between two functions. We illustrate \parseval's identity for three inputs, which can easily be generalized for an arbitrary number of inputs. \Cref{sec:complete-construction} leverages these considerations to build the $n$-\players \sysname protocol.

Firstly we note that in case of two \players Parseval's identity may be cast into the following form
\begin{align}\label{eq:gpar2-3ainputs}
&\frac{1}{2}a_0\alpha_0+\frac{1}{2}\boldsymbol{(A+B)\cdot(\alpha+\beta)}+\frac{1}{2}\boldsymbol{(A-B)\cdot(\alpha-\beta)}=\nonumber \\
&\frac{1}{l}\int_{-l}^l f(x)g(x)dx
\end{align}
Let's now consider three inputs,  $f(x)$, $g(x)$ and $h(x)$ with \fourier series representations given by \Cref{eq:conv1} and by
\begin{equation}\label{eq:gpar1}
h(x)=\frac{\gamma_0}{2}+\sum_{n=1}^\infty \gamma_n\cos\bigl(\frac{n\pi}{l}x\bigr)+\sum_{n=1}^\infty \varrho_n\sin\bigl(\frac{n\pi}{l}x\bigr)\\ 
\end{equation}
respectively; the generalized \parseval's identity reads:
\begin{align}\label{eq:gpar2-3inputs}
&\frac{1}{2}a_0\alpha_0\gamma_0+ \frac{1}{2}\boldsymbol{(A+B)\cdot(\alpha+\beta)\cdot(\gamma+\varrho)} +\\ \nonumber
&\frac{1}{2}\boldsymbol{(A-B)\cdot(\alpha-\beta)\cdot(\gamma-\varrho)}= \\ \nonumber
& \frac{1}{l}\int_{-l}^lf(x)(g\star h)(x)dx+\frac{1}{l}\int_{-l}^lg(x)(f\star h)(x)dx+
\\ \nonumber 
&\frac{1}{l}\int_{-l}^lh(x)(f\star g)(x)dx-\frac{2}{l}\int_{-l}^l\hat{h_c}(x)(\hat{f_c}\star \hat{g_c})(x)dx
\end{align}
or
\begin{align}\label{eq:gpar3}
&\frac{a_0\alpha_0 \gamma_0}{2}+\frac{1}{2}\sum_{n=1}^\infty (a_n+b_n)(\alpha_n+\beta_n)(\gamma_n+\varrho_n)+
\\ \nonumber
&\frac{1}{2}\sum_{n=1}^\infty (a_n-b_n)(\alpha_n-\beta_n)(\gamma_n-\varrho_n)= \\ \nonumber
& \frac{1}{l}\int_{-l}^lf(x)(g\star h)(x)dx+\\ \nonumber
&\bigg(\frac{1}{l}\int_{-l}^lg(x)(f\star h)(x)dx-\frac{1}{l}\int_{-l}^l\hat{g_c}(x)(\hat{f_c}\star \hat{h_c})(x)dx\bigg) +\\ \nonumber
\\ \nonumber 
&\bigg(\frac{1}{l}\int_{-l}^lh(x)(f\star g)(x)dx-\frac{1}{l}\int_{-l}^l\hat{h_c}(x)(\hat{f_c}\star \hat{g_c})(x)dx\bigg)
\end{align}\label{eq:gpar4}
Vectors $\bold A$, $\bold B$, $\boldsymbol{\alpha}$, $\boldsymbol{\beta}$ and $\boldsymbol{\gamma}$ and $\boldsymbol{\varrho}$ are respectively defined as
\begin{align}\label{eq:gpar5}
{\bf A}&=\{a_n\} \ \  ; \ \  {\bf B}=\{b_n\} \quad (n=1,2,\cdots) \\ \nonumber
{\boldsymbol\alpha}&=\{\alpha_n\}\ \ ;\ \ {\boldsymbol\beta=\{\beta_n\}}\quad(n=1,2,\cdots)\\ \nonumber
{\boldsymbol\gamma}&=\{\gamma_n\}\ \ ;\ \ {\boldsymbol\varrho=\{\varrho_n\}}\quad (n=1,2,\cdots)
\end{align}
and 
\begin{align}\label{eq:gpar6}
\hat{f}_c(x)&\equiv\frac{1}{2}\Bigl(f(x)+f(-x)\Bigr) \ \  ; \  \hat{g}_c(x)\equiv\frac{1}{2}\Bigl(g(x)+g(-x)\Bigr) \nonumber\\
\hat{h}_c(x)&\equiv\frac{1}{2}\Bigl(h(x)+h(-x)\Bigr)
\end{align}
A mathematical formula for an arbitrary number of inputs can easily be obtained by performing similar calculations. 

==> sections/security.tex <==
% =========
% security 
% =========

